AutoFreeze: Automatically Freezing Model Blocks to Accelerate Fine-tuning

With the rapid adoption of machine learning (ML), a number of domains now use the approach of fine tuning models which were pre-trained on a large corpus of data. However, our experiments show that even fine-tuning on models like BERT can take many hours even when using modern accelerators like GPUs. While prior work proposes limiting the number of layers that are fine-tuned, e.g., freezing all layers but the last layer, we find that such static approaches lead to reduced accuracy. We propose, AutoFreeze, a system that uses an adaptive approach to choose which layers are trained and show how this can accelerate model fine-tuning while preserving accuracy. We also develop mechanisms to enable efficient caching of intermediate activations which can reduce the forward computation time when performing fine-tuning. We extend AutoFreeze to perform distributed fine-tuning and design two execution modes that minimize cost and running time respectively. Our evaluation on ten NLP tasks shows that AutoFreeze, with caching enabled, can improve fine-tuning on a single GPU by up to 2.55x. On a 64 GPU cluster, for fine-tuning on the AG's news dataset, AutoFreeze is able to achieve up to 4.38x speedup when optimizing for end-to-end training time and 5.03x reduction in total cost when optimizing for efficiency, without affecting model accuracy.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}
Developing ML models for new tasks is challenging and thus a number of tasks are bootstrapped with features or weights from existing models.
This includes transfer learning~\cite{sharif2014cnn}, where features from a large pre-trained model are used on a new task and only the last few layers are trained to develop a specialized model. Closely related is the practice of fine tuning where weights from a pre-trained model are used to initialize training for a new task. Following initialization all layers of the model are trained until convergence. Model fine-tuning has been shown to achieve high accuracy: for example, fine-tuning Bidirectional Encoder Representations from Transformers (BERT) \cite{devlin2018bert}, a pre-trained language representation model, has been shown to achieve state-of-the-art results on several natural language processing (NLP) tasks such as sentiment analysis~\cite{maas-etal-2011-learning}, topic classification~\cite{zhang2016characterlevel} etc. In addition to the accuracy benefits, fine-tuning also reduces training resources required. For example, training BERT from scratch can take up to 4 days even when using 4 Cloud TPUs~\cite{devlin2018bert}.

With a number of ML tasks using the above approach, we investigate the time and resources required for fine-tuning. 
We find that even fine-tuning for a few epochs can takes several hours even with the use of GPUs. This is primarily because the pre-trained models are often very computation-heavy, e.g., running one epoch of fine tuning on $BERT_{BASE}$ model, for Yelp dataset (650K data points) takes around 13 hours on a NVIDIA P100 GPU.\shivaram{While this can be accelerated by performing distributed fine-tuning using a cluster of GPUs, this incurs additional costs making it prohibitive for repeated fine-tuning that is required as datasets evolve over time~\cite{something?}}



\begin{figure}
\includegraphics[width=\linewidth]{figures/timeline.pdf}
  \caption{We present a high level design of \sys{}. During fine-tuning, \textbf{\sys{}} adaptively determines layers which can be frozen. Once layers are frozen, the backward computation for those layers can be avoided. At later epochs, intermediate outputs are also cached leading to further gains. }
  \label{fig:timeline}
\end{figure}






A natural approach to improve fine-tuning performance is to limit the number of layers of the model that are updated, thus making it similar to transfer learning. 
For example, if we consider BERT$_{BASE}$ which has 12 encoding blocks, prior approach in~\cite{lee2019would} trains a fixed number of blocks (e.g., the last 4 blocks) and \emph{freezes} the weights for the remaining blocks. However, this approach can affect the final model accuracy. For example with the IMDb dataset~\cite{maas-etal-2011-learning} this approach can reduce the time for an epoch by 65\%, but we find that the accuracy of the fine-tuned model suffers, dropping from 93.94\% to 92.2\%. Another approach used in prior work~\cite{chen2020lottery} is to apply the ``Lottery Ticket Hypothesis'' to identify matching subnetworks in pre-trained BERT models to enforce sparsity in models trained for different downstream tasks. While this approach retains accuracy and can lead to sparser models, it does not lead to improvements in training speed without dedicated hardware/libraries\cite{liu2018rethinking}.
%\shivaram{can we cite something to make this claim?}

In this paper we propose an improved approach where the number of model blocks that are updated during fine-tuning are adaptively chosen during the fine-tuning process. Our work is inspired by recent work of \citep{Raghu2017SVCCASV} who developed SVCCA, a new metric that captures how different layers of model change over the course of training. The SVCCA score for a layer, as proposed in~\cite{Raghu2017SVCCASV}, is computed by comparing the intermediate model weights with the final weights and can thus be used for post-hoc analysis.  Applying that approach to model fine-tuning we observe that the initial layers of the model converge rapidly and thus we can \emph{freeze} such layers. Freezing the initial layers means that the backward pass for those layers can be skipped, thereby reducing the computation required. While SVCCA scores show the promise of freezing layers early, we still need an online algorithm that can decide which layers should be frozen and when. We develop a gradient-norm based test that ranks layers by their rate of change and based on the selects the slowest changing layers for freezing. We show that our test is effective at detecting when layers should can be frozen without affecting accuracy across multiple datasets.

\shivaram{Lets modify this paragraph to talk about distributed fine-tuning} Freezing early layers of a model can reduce the time taken by the backward pass, but we still need to do the forward pass corresponding to the frozen layers as shown in Figure~\ref{fig:timeline}. For a model like $BERT_{BASE}$ we find that even running just the forward pass can take 550 seconds per epoch with the IMDb dataset (Figure~\ref{fig:freeze_potential_benefits_imdb}).  We can further reduce the training time by using the observation that once model layers are frozen, then for a given data point, the output of the forward pass will remain the same across different epochs of training. Thus, along with freezing we can also \emph{cache} the output of the forward pass up to the layer that has been frozen. Once the same data point is selected to be used again for training, we can load the pre-computed intermediate values from our cache and continue training. \yuhan{In the distributed fine-tuning setup, freezing can reduce the gradient size to be aggregated among workers, leading to both computation and communication improvements. }

\shivaram{and also this part needs to be changed.}
We design \sys{}, a system for automatically freezing model blocks to accelerate fine-tuning. 
Our system consists of two main modules on each GPU: a \emph{freezing module} that has a pluggable decision engine that can make decisions on which layers should be frozen as training progresses. In the distributed fine-tuning setup, the decision is made on the gradients aggregated among workers. We also design a \emph{storage manager} to implement the caching functions described above. The storage manager handles a number of common concerns in caching, including selecting the appropriate backend (CPU memory / SSD etc.) and deciding when to evict data from the cache. In addition, we observe that typically, the order in which data points are accessed varies across epochs. The storage manager takes into account the ordering of data access in future epochs to layout data in appropriate order when storing. \yuhan{Made some edits. } 



We evaluate \sys{} using a wide range of fine-tuning tasks.
% including topic classification on the AG's News dataset~\cite{zhang2016characterlevel} and Sogou News dataset\cite{sun2019fine}, sentiment analysis on Yelp Full dataset\cite{zhang2016characterlevel} and IMDb dataset\cite{maas-etal-2011-learning}, question answering on SQuAD2.0 dataset\cite{rajpurkar2018know}, multiple choice task on SWAG dataset\cite{zellers2018swag}, and text summarization on CNN/DailyMail dataset \cite{hermann2015teaching}. 
We find that \sys{} can improve training time by up to 2.55$\times$ while affecting accuracy by less than 0.1\%. We also show that \sys{} is especially effective  for large datasets like Yelp where freezing layers reduces fine-tuning time from 52.5 hours to 27 hours and caching further reduces this to 24.6 hours. \yuhan{Applying \sys{} in distributed fine-tuning can reduce the end-to-end training time from 11271 seconds to 2573 seconds for training AG's News dataset on 64 machines. }


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/freezing_gains_imdb.pdf}
    \caption{\small{\textbf{Potential Benefits of Freezing:} For IMDb dataset we show the potential savings in time when performing freezing. Time for forward pass is constant since we need to perform a full forward pass before calculating gradients. On the other hand timing for backward pass reduces as we increase number of layers frozen.}}
    \label{fig:freeze_potential_benefits_imdb}
    \vspace{-0.2in}
\end{figure}
